EgoXperience: Learning World-Grounded Egocentric Representations from Human Experience

Reconstructing human activity from egocentric video requires more than recovering individual 3D components: the observer's motion, surrounding geometry, and hand-object interactions must fit together in a consistent world. Achieving this coherence requires both joint reconstruction and aligned supervision, yet existing methods and datasets offer limited support for either. We present EgoXperience, a full-stack paradigm that addresses these needs through data collection, automatic annotation, unified modeling, and benchmarking. Central to EgoXperience is an automatic annotation engine, EgoX-Engine, that couples geometrically verified object tracking with SLAM-based world alignment, yielding consistent supervision for the camera, scene, hands, and objects. This yields EgoX-Data-6M, a 50-hour dataset of task-driven manipulation and locomotion within and across indoor and outdoor environments, with second-level task captions. We carefully select one hour across these activity categories as EgoX-Bench to evaluate joint reconstruction. To translate this supervision into reconstruction, we introduce EgoX, trained with EgoX-Data-6M and complementary annotations from additional public datasets. Given monocular egocentric video and first-frame object masks, our model achieves joint metric reconstruction of the camera, scene, hands, and objects in a shared world coordinate frame with a single forward pass. Extensive experiments demonstrate state-of-the-art performance across scene estimation and world-space hand-object pose recovery. Against the strongest evaluated baselines, EgoX reduces camera, hand, and depth errors by 68.9%, 65.6%, and 42.9%, and improves object pose scores by 28.0%.

==> tabs/ropedia_dataset_summary.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ropedia/Xperience Dataset Summary.}
Replace the row values with the statistics of the target Ropedia release.
}
\label{tab:ropedia_dataset_summary}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l >{\columncolor{subcol}}c c >{\columncolor{subcol}}c c >{\columncolor{subcol}}c c c c >{\columncolor{subcol}}r}
\toprule
\textbf{Dataset}
& \textbf{Environment}
& \textbf{Dynamics}
& \textbf{View Type}
& \textbf{Source}
& \textbf{Single}
& \textbf{Sparse}
& \textbf{Medium}
& \textbf{Dense}
& \textbf{\#Frames} \\
\midrule
Xperience~\citep{xperience_10m} & Indoor & Dynamic & Egocentric & Real & 2 & 2 & 2 & 2 & 3{,}089 \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tabs/ropedia_results_template.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ropedia Per-Regime Results Template.}
Report depth, pose, trajectory, or task-specific metrics under the regimes used by the paper.
Best values can use \colorbox{rankfirst}{deep green}, second-best values \colorbox{ranksecond}{medium green}, and third-best values \colorbox{rankthird}{light green}.
}
\label{tab:ropedia_results_template}
\resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.12}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c >{\columncolor{subcol}}c c >{\columncolor{subcol}}c c >{\columncolor{subcol}}c c}
\toprule
\multirow{2.5}{*}{\textbf{Method}}
& \multirow{2.5}{*}{\makecell{\textbf{\#Params}\\\textbf{(M)}}}
& \multicolumn{2}{c}{\textbf{Sparse}}
& \multicolumn{2}{c}{\textbf{Medium}}
& \multicolumn{2}{c}{\textbf{Dense}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
& & AbsRel$\downarrow$ & AUC@30$\uparrow$ & AbsRel$\downarrow$ & AUC@30$\uparrow$ & ATE$\downarrow$ & Success$\uparrow$ \\
\midrule
Baseline A & -- & \cellcolor{rankthird}0.120 & \cellcolor{rankthird}0.420 & \cellcolor{rankthird}0.095 & \cellcolor{rankthird}0.460 & \cellcolor{rankthird}1.800 & \cellcolor{rankthird}0.620 \\
Baseline B & -- & \cellcolor{ranksecond}0.090 & \cellcolor{ranksecond}0.540 & \cellcolor{ranksecond}0.075 & \cellcolor{ranksecond}0.580 & \cellcolor{ranksecond}1.250 & \cellcolor{ranksecond}0.740 \\
\ours (Ours) & -- & \cellcolor{rankfirst}\textbf{0.060} & \cellcolor{rankfirst}\textbf{0.680} & \cellcolor{rankfirst}\textbf{0.052} & \cellcolor{rankfirst}\textbf{0.710} & \cellcolor{rankfirst}\textbf{0.820} & \cellcolor{rankfirst}\textbf{0.860} \\
\bottomrule
\end{tabular}%
}
\end{table}

